A Modular Structural Operational Semantics for Delimited Continuations

It has been an open question as to whether the Modular Structural Operational Semantics framework can express the dynamic semantics of call/cc. This paper shows that it can, and furthermore, demonstrates that it can express the more general delimited control operators control and shift.

==> eptcsdata.tex <==
\providecommand{\firstpage}{63}
\providecommand{\publicationstatus}{Olivier Danvy \& Ugo de'Liguoro (Eds.):
WoC'15 Postproceedings\\
EPTCS 212, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.212.5}{10.4204/EPTCS.212.5}}

